Tropical (1, 1)-homology for floor decomposed surfaces

The tropical (p, q)-homology groups of Itenberg, Katzarkov, Mikhalkin and Zharkov are the tropical analogues of the Hodge decomposition of the cohomology of complex algebraic varieties. There is a well-defined intersection pairing on tropical (1, 1)-classes of a compact non-singular tropical surface. Here we compute directly the (1, 1)-homology of a non-singular floor decomposed tropical surface in tropical projective space, along with the intersection form.

==> intersection.tex <==



\begin{section}{Intersection form on $H_{1, 1}$}\label{sec:intersection}



\begin{example}
To start with consider the basic example of a floor decomposed quadric surface $S$. Its floor plan is a pair of curves $L$,  a line,  and $C$, a conic. 
%By Section \ref{sec:groups}, $H_{1, 1} = \Z^2$. 
Figure \ref{fig:-2cycle} shows the floor plan along with a part of the surface $S$. The union of the curves
 $L \cup C$ contains a cycle drawn in red, let it be oriented so that it is the boundary of the bounded cell. Now equip the corresponding $1$-cycle in $S$ with a 
 vertical framing and call it $\sigma$. Without the framing  this cycle is of course homologous to zero, however $\sigma \in Z_{1, 1}$ cannot be contracted 
in the same way since the vertical direction is not contained in the bounded face of which the cycle is the boundary.

Moving the cycle $\sigma$ into the interior of the vertical faces as in Figure \ref{fig:-2cycle}, it is still forced to pass through two vertices of the surface. 
Each point contributes $-1$ to the self intersection of $\sigma$, so $\sigma^2 = -2$. 
It is possible to choose a hyperplane section which does not intersect the $(1, 1)$-cycle $\sigma$. 
So we obtain the intersection matrix $$Q(S_2) = \left(\begin{array}{cr}2 & 0 \\0 & -2\end{array}\right).$$
\end{example}

\vspace{0.5cm}

In part, the general situation is similar to what is described above. 
Let $S$ be a floor decomposed surface  of degree $d$ in $\TP^3$ given by the sequence of curves $C_1, \dots , C_d \subset \R^2$. 
The $1$-skeleton of a floor corresponding to a pair of curves $C_i, C_{i+1}$ supports $g(2i + 1)$ independent $1$-cycles. Equip  these
with a constant upward vertical framing to obtain $(1, 1)$-cycles. A $(1, 1)$-cycle  supported 
on just one of the two curves, $C_i, C_{i+1}$ can be translated vertically off of the floor,  (upwards or downwards, depending if it is on $C_i$ or $C_{i+1}$). 


For a floor, we use the term \textit{junction} for an intersection point of the two curves defining the floor, ie, a point in $C_{i-1}\cap C_i$, of which there are $(i-1)i$.  Every $(1, 1)$-cycle $\alpha$ given by a $1$-cycle on the skeleton with vertical framing determines a function on the junctions, 
$$\delta_{\alpha}: C_{i-1} \cap C_i \longrightarrow \{-1, 0, 1\},$$ by 
%
%\begin{eqnarray*}
$$\delta_{\alpha}(x) =   \left\{ 
\begin{array}{l l}
  0&  \quad \mbox{if $x \not \in \alpha$ or  $\alpha$ goes from $C_i$ to $C_i$ through $x$}\\
  1&  \quad \mbox{if $\alpha$ is oriented from  $C_i$ to $C_{i-1}$ through $x$ }\\ 
  -1 &     \quad \mbox{if $\alpha$ is oriented from $C_{i-1}$ to $C_{i}$ through $x$ }
  \end{array} \right. $$
%\end{eqnarray*}




\begin{proposition}\label{prop:IntPairing}
The boundary of a horizontal bounded cell in a floor decomposed surface equipped with upward vertical framing is a $(1, 1)$-cycle. Moreover, two such $(1, 1)$-cycles  $\alpha$, $\beta$  satisfy,  
\begin{enumerate}
\item $\alpha^2 = - \sum_{x \in C_d \cap C_d-1} \delta_{\alpha}(x)^2 $ 
\item $\alpha.\beta =  - \sum_{x \in C_d \cap C_d-1} \delta_{\alpha}(x)\delta_{\beta}(x)$. 
\item $H. \alpha = 0$ where $H$ is a hyperplane section. 
\end{enumerate}
\end{proposition}


\begin{proof}
If the edges of the boundary are oriented so that they form a simplicial cycle then we have a $(1, 1)$-cycle because the framing is constant. 

Such a $(1,1)$-cycle $\alpha$ may be continuously deformed as in Figure \ref{cycleHyper}.
An edge of $\alpha$ on $C_d$ can only be slid downwards and an edge on $C_{d-1}$ can be slid upwards, leaving the cycle to pass through the junction points if $\delta_{\alpha}(x) \not =0$. There  is an integral affine map taking a neighborhood of a junction to the standard hyperplane and sending the deformed $\alpha$ and $\beta$ to cycles presented in  Example \ref{ex:pqMinus1}.  If $\delta_{\alpha}(x) = 1$ then the framing is consistent with the orientation of the cell at the junction point, if it is $-1$ then the framing is opposite. Example  \ref{ex:pqMinus1} calculates the intersection product for pairs of such cycles to be $$-\delta_{\alpha}(x)\delta_{\beta}(x).$$  The assumption that all cycles have an upward vertical framing is crucial.  This proves $(2)$. 
Statement $(1)$ is just a  special case of $(2)$, it is just to emphasise that each junction with $\delta_{\alpha}(x) \not = 0$ contributes $-1$ to the self intersection of $\alpha$.

For $(3)$, there is a tropical  plane $P$ which intersects none of these $(1, 1)$ cycles supported on the floors. Simply  take $P$ to be a translate of the standard plane centered at the origin by $Mv$ for $M >>0$ and $v$ a generic vector choice of vector in $\R^n$. 
\end{proof}


Ignoring these for now and consider the remaining $$g(2i+1) - g(i+1) -g(i) = i(i-1)-1$$ cycles. 
The intersection form restricted to these cycles is the matrix of dimension $i(i-1)-1$:


\[
 Q_{i} =\left(
 \begin{array}{rrrrr}
  -2 & 1   & \\
  1& -2 & 1 & \\
   &  1 & -2 &    \ddots   \\
     &  & \ddots & \ddots & 1      \\
   & &  & 1 & -2
 \end{array} \right)
\]

This is easy to see once the appropriate basis is fixed. Choose any labeling of the $(i-1)i$ junction points of $C_i, C_{i-1}$ and for $1 \leq k \leq i(i-1)-1$ let the cycle $\sigma_k$ be a cycle on $(C_i \cup C_{i-1})^{(1)}$ for which $\delta_{\sigma_k}(x_k) = 1, \delta_{\sigma_k}(x_{k+1}) = -1,$ and  $\delta_{\sigma_k}(x_l) = 0$ otherwise. 


\begin{figure}
\includegraphics[scale=0.3]{figures/2floorplan.jpg}
\hspace{2cm}
\includegraphics[scale=0.6]{figures/-2cycle.pdf}
\caption{ A $-2$ cycle on a floor (L, C)}
\label{fig:-2cycle}
\end{figure}

\comment{
\begin{subsection}{Intersection form on $(2, 0)$ and $(0, 2)$ classes}
Refer to the example of the case of curves. 
\end{subsection}}


\end{section}
